Characterisation of Strongly Normalising lambda-mu-Terms

We provide a characterisation of strongly normalising terms of the lambda-mu-calculus by means of a type system that uses intersection and product types. The presence of the latter and a restricted use of the type omega enable us to represent the particular notion of continuation used in the literature for the definition of semantics for the lambda-mu-calculus. This makes it possible to lift the well-known characterisation property for strongly-normalising lambda-terms - that uses intersection types - to the lambda-mu-calculus. From this result an alternative proof of strong normalisation for terms typeable in Parigot's propositional logical system follows, by means of an interpretation of that system into ours.

==> Macros.tex <==
% { ( [
% Format commands
\newskip \point \point=1pt
\makeatletter

%\def\Vec#1{\overrightarrow{#1}}

\newlength\harpoonlength

%\def \longharpoon#1{\psset{unit=1pt,linewidth=0.35pt}\psline{cc-cc}(0,1.5)(#1,1.5)\hspace*{#1}\pscurve{cc-cc}(0,1.5)(-1.1,2)(-1.75,2.75)\hspace*{.1#1}}
\def \longharpoon#1{\harpoonlength#1%\advance\harpoonlength-1pt
\psset{unit=1pt,linewidth=0.35pt}\psline{cc-cc}(1,1.25)(\harpoonlength,1.25)\hspace*{\harpoonlength}\pscurve{cc-cc}(0,1.25)(-1.1,1.75)(-1.75,2.5)\hspace*{.1\harpoonlength}}

\newcommand{\Vec}[2][]{%
\setbox155=\hbox{${#2}$}%
\setbox156=\hbox{$_{#1}$}%
\leavevmode
\ifdim\wd155<6\point\setbox155=\hbox{$\hspace{1\point}#2\hspace{1\point}$}\fi
\ifdim\ht155>5.5\point
{\raise\ht155\hbox{\longharpoon{\wd155}}}\else
{\raise5.5\point\hbox{\longharpoon{\wd155}}}\fi
\kern-1.1\wd155% put argument and move left
\ifdim\wd156<2pt\box155\else\box155\box156\fi}


%\newcommand{\Proof}{\noindent {\it Proof.}~}

\def \QED {~\hfill\hbox{\rule{5.5pt}{5.5pt}\hspace*{.5\leftmarginii}}}

\def \hskp {\hspace*{.75\point}}
\def \skp {\hspace*{1.5\point}}
\def \Skip	{\hspace*{3.5\point}}
\def \Set#1{\{\hskp #1 \hskp\}}
\def \Pred[#1]{\,[\hskp #1 \hskp]}
\def \Exists{\exists\,}
\def \Forall{\forall\,}
\def \IH {\textrm{\it IH}}
\def \And{\mathrel{\&}}
\def \Weak{\textrm{\it W}}
\def \Par{\mathop{\mid}}

\newcommand{\Power}[1]{{\cal P}(#1)}
\newcommand{\der}{\vdash}
% \newcommand{\Nat}{\mathbb{N}} % natural numbers

\def \Natural{\ensuremath{%
\hbox{\psset{unit=.0725em,linewidth=.5}%
\psline{-}(3.35,0)(3.35,8)}{\sf N}}}
\def \Nat{\Natural}

\newcommand{\NF}{{\cal N}}

% Meta logic

\newcommand{\Implies}{\Rightarrow}
\newcommand{\dom}{\textrm{\it dom}}
\def\to{\mathbin{\mapsto}}
\def \Union {\mathrel{\cup}}
\def \Dom(#1){\textit{dom}\,(#1)}
\def\cons{\mathop{:}}
\def\becomes{\mathop{:=}}


% Lambda-Mu calculus syntax

\newcommand{\Terms}{\mbox{\sf \small Trm}}
\newcommand{\Commands}{\mbox{\sf \small Cmd}}
\newcommand{\Cmd}{\mbox{\sf \small C}}
\newcommand{\Formulas}{\textbf{LF}}

\newcommand{\StrSub}[2]{[#1 \Becomes #2]}%{[#1 \Becomes #3{`.}#2]}  % \StrSub{\alpha}{N} = structural substitution of [\alpha]L by [\alpha]LN
%\def \strSub [#1 <= #2.#3]{[#1 \Becomes #2{`.}#3]} 
%\def \strSubvec [#1 <= #2.#3]{[#1 \Becomes \Vec{#2{`.}#3}]} 
\def \strSub [#1<=#2]{[#1 \Becomes #2]} 
\def \strSubvec [#1<=#2]{[#1 \Becomes \Vec{#2}]} 
\def \scstrSubvec [#1<=#2]{[#1 \Becomes {\mbox{\scriptsize $#2$}}]} 
\newcommand{\StrSubNoB}[2]{#1 \Becomes #2}  % structural substitution without brackets
\newcommand{\reduces}{\rightarrow} % one step reduction
\newcommand{\Rename}{\textrm{\it ren}} % renaming reduction rule
\newcommand{\TVar}{\textrm{\it Var}}
\newcommand{\CVar}{\textrm{\it Name}}
\newcommand{\LamMuTerm}{\Lambda\mu\textsf{-Trm}}
\newcommand{\LamMuTheory}{\Lambda\mu}
\newcommand{\ExtLamMuTheory}{\Lambda\mu\eta}
\newcommand{\derLM}{\der_{\Lambda\mu}}
\newcommand{\derLME}{\der_{\Lambda\mu\eta}}
\newcommand{\convLM}{=_{\Lambda\mu}}
\newcommand{\convLME}{=_{\Lambda\mu\eta}}

%\newcommand{\Tran}[1]{\overline{#1}}
\newcommand{\CPS}[1]{\underline{#1}}

\newcommand{\SN}{{\cal S}\kern-1\point {\cal N}}

% Types
\newcommand{\Types}{\textsf{Type}}

\def\length#1{{\mid}#1{\mid}}

\newcommand{\typeJudg}[3]{\derLmu {#1} |- {#2} | {#3} } % judgment:  Gamma (#1) |- M:sigma (#2) | Delta (#3)
\newcommand{\Axiom}{\textrm{\it Ax}} 
\newcommand{\arrowE}{\arrow\textrm{\it E}}
\newcommand{\arrowI}{\arrow\textrm{\it I}}
\newcommand{\botI}{\bot}
\newcommand{\muI}{\mu}
\newcommand{\intersI}{\inters}
\newcommand{\omegaI}{\omega}
\newcommand{\leqI}{\leq}
\def \leqA	{\mathrel{\leq_A}}
\def \leqC	{\mathrel{\leq_C}}
\def \leqD	{\mathrel{\leq_D}}
\def \union	{\mathrel{\cup}}


\newcommand{\eraseT}[1]{\mid\!\! #1 \!\!\mid}

%\newcommand{\arrow}{\rightarrow}
\newcommand{\TypeTheor}{{\cal T}}

\newcommand{\Lang}{{\cal T}}

% Semantics
\newcommand{\TypeSem}[1]{\|#1\|}
\def\TSem{\TypeSem}

\newcommand{\SemArrow}{\rightarrow}

\newcommand{\Env}{\textsf{Env}}

\newcommand{\Domain}{{\cal D}}
\newcommand{\comp} { {\,\circ\,} }
\newcommand{\Isom}{\simeq}
\def\PairBr<#1,#2>{\langle #1,\skp #2 \rangle}
\def\PairNoBr#1#2{\langle #1,\, #2 \rangle}
\def\Pair{\@ifnextchar<{\PairBr}{\PairNoBr}}
% \newcommand{\Pair}[2]{\langle #1,\, #2 \rangle}
\newcommand{\UPair}[2]{\langle #1, #2 \rangle}

\newcommand{\Stop}{\textsf{stop}}

\newcommand{\PairComb}{\mbox{\bf P}}
\newcommand{\ProjComb}[1]{\PairComb_{#1}}
\newcommand{\Eval}{\textsf{eval}}
%\newcommand{\Abs}{\textsf{abs}}

\newcommand{\Filt}{{\cal F}}
%\newcommand{\App}[2]{#1  \cdot #2}

\newcommand{\SuperOp}{\mbox{\it\footnotesize op}}
\newcommand{\Compact}{{\cal K}}
\newcommand{\CompOp}{\Compact^{\SuperOp}}

\newcommand{\ALG}{\mbox{\rm \bf ALG}}

\newcommand{\Rank}{\textrm{\it rk}\,}
\newcommand{\StepFun}[2]{(#1 \Rightarrow #2)}
\newcommand{\Filter}{\textsf{Filt}}

\newcommand{\TypeToComp}{\Theta}
\newcommand{\normalForm}{\textrm{\it nf}\,}
\newcommand{\TypeTransl}{\Phi}

\newcommand{\Idnt}{\textsf{Id}}

\def\Ax{\textrm{\it ax}}
\def\arrE{{\rightarrow}\textrm{\it E}}
\def\arrI{{\rightarrow}\textrm{\it I}}
\def\quaE{{\forall}\textrm{\it E}}
\def\quaI{{\forall}\textrm{\it I}}
\def\intI{{\inter}I}
\def\inter{\mathord{\wedge}}
\def\prod{\mathord{\times}}
\def\arrow{\mathord{\rightarrow}}
\def\inters{\inter}
\def\red{\rightarrow}
\def \Becomes{\mathop{\Leftarrow}}
\def\same{\equiv}
\def\Then{\mathrel{\Rightarrow}}
\def\If{\mathrel{\Leftarrow}}
\def \Iff	{\mathrel{{\Leftarrow}\kern-5\point{\Rightarrow}}}
\def \k	{\underline{k}}
\def \n	{\underline{n}}
\def \m	{\underline{m}}
\def \r	{\underline{r}}
\def \ele {\mathbin{\in}}
\def \notele {\mathrel{\not\nobreak\in}}
\def\dotn{`d_i\,(i\ele\n)}
\def \FV#1{\textrm{\it fv}\skp({#1})}
\def \fv(#1){\FV{#1}}
\def \FN#1{\textrm{\it fn}\skp({#1})}
\def \fn(#1){\FN{#1}}
%\newcommand{\fn}{\textrm{\it fn}}
%\newcommand{\fv}{\textrm{\it fv}}

\setbox138=\hbox{$=$}
\setbox139=\hbox{{\scriptsize $\Delta$}}%
\setbox149=\hbox{\raise-1\point\copy138\kern-.5\wd138\kern-.5\wd139\raise5\point\hbox{\copy139}\kern-.5\wd139\kern.5\wd138}
\def \ByDef {\mathrel{\copy149}}

\def \cont{\mbox{\small \sf C}}
\def\ContP'{\cont'\hskp}
\def\Cont{\@ifnextchar'{\ContP}{\cont\hskp}}

\def \LeftTop#1{\hspace{2\point}%\leavevmode\kern2\point
\setbox66=\hbox{$#1$}%
\ifdim\ht66>5\point \setlength{\unitlength}{.2\point} 
	\psset{unit=.135\ht66,linewidth=0.4\point,linecolor=black}%
\else \setlength{\unitlength}{.2\point} 
	\psset{unit=.8\point,linewidth=0.4\point,linecolor=black}%
\fi
\ifmycolour\psset{linecolor=semcolour}\fi
\setbox67=\hbox{\put(0,4)%
{\psline{c-c}(0,0)(3,0)%
 \psline{cc-cc}(0,0)(0,-8)%
 \psline{cc-cc}(1.5,0)(1.5,-6)%
}}%
\raise7.25\point\box67%\fi 
\kern3\point{#1}}

\def \RightBot{\kern2.75\point
\psset{unit=1.2\point,linewidth=0.4\point,linecolor=black}%
\ifmycolour\psset{linecolor=semcolour}\fi
\hbox{\put(2.5,-10)%
{\psline{c-c}(0,0)(-3,0)%
 \psline{cc-cc}(-1.35,0)(-1.35,6)%
 \psline{cc-cc}(0,0)(0,8)%
}}\kern2.5\point}

\def\USem{\SEM}
\def\Sem{\SEM}
%\def\SemPr#1{\LeftTop{#1}\RightBot}
\def\SemPr#1{[\kern-1.6\point[{#1}]\kern-1.6\point]\kern-.5\point}

\def \SemTwo#1#2{\SemPr{#1}\skip{#2}}
\def \SemThree#1#2#3{\SemPr{#1}\Skip{#2}\Skip{#3}}
\def \SemSOne#1#2{\SemPr{#1}\kern-1\point^{#2}}
\def \SemSTwo#1#2#3{\SemPr{#1}\kern-1\point^{#2}\skip{#3}}
\def \SemSThree#1#2#3#4{\SemPr{#1}\kern-1\point^{#2}\Skip{#3}\Skip{#4}}

\def \SemNoSTwo#1#2{\@ifnextchar\bgroup{\SemThree{#1}{#2}}{\SemTwo{#1}{#2}}}
\def \SemNoS#1{\@ifnextchar\bgroup{\SemNoSTwo{#1}}{\SemPr{#1}}}
%
\def \SemSNotOne#1#2#3{\@ifnextchar\bgroup{\SemSThree{#1}{#2}{#3}}{\SemSTwo{#1}{#2}{#3}}}
\def \SemS#1^#2{\@ifnextchar\bgroup{\SemSNotOne{#1}{#2}}{\SemSOne{#1}{#2}}}
\def \SemBr[#1]{\@ifnextchar^{\SemS{#1}}{\SemNoS{#1}}}
\def \SemNoBr#1{\@ifnextchar^{\SemS{#1}}{\SemNoS{#1}}}
\def \SEM{\@ifnextchar[{\SemBr}{\SemNoBr}}%]

\def \turn	{{\vdash}}
\def \Turn	{\mathbin{\vdash}}
\def \TurnL	{\mathbin{{\vdash}\kern-1\point_{`l}}}
\def \TurnLmu {\Turn}%{\mathrel{\turn\kern-\point_{`l`m}}}
\def \TurnP {\mathbin{{\vdash}_{\kern-2\point\textsc {\scriptsize p}}}}
\def \TurnR {\mathbin{{\vdash}_{\kern-2\point\textsc {\scriptsize r}}}}
\def \Mid{\hspace*{2.5pt}{\black \mid}\hspace*{2.5pt}}
\def \lstat#1#2{{#1}\,{:\,}{#2}}

\def \Stoup#1#2{\lstat{#1}{#2}}
\def \StoupR#1#2{\lstat{#1}{#2} \Mid}
\def \StoupR#1#2{\framebox{$#1\,{:}\,#2$}~}
\def \StoupR#1#2{\StoupFrame{\lstat{#1}{#2}}}
\def \StoupL#1#2{\StoupFrameL{\lstat{#1}{#2}}}
%
\def \Stoup#1#2{\lstat{#1}{#2}}
\def \StoupL#1#2{\Mid\Skip\lstat{#1}{#2}}
\def \StoupR#1#2{\lstat{#1}{#2}\Skip\Mid}
%
\def \DerLmuThree#1#2#3{#1 \TurnLmu \Stoup{#2}{#3} }
\def \DerLmuFour#1#2#3#4{#1 \TurnLmu \StoupR{#2}{#3} #4}
\def \DerLmu#1#2#3{\@ifnextchar{\bgroup}{\DerLmuFour{#1}{#2}{#3}}{\DerLmuThree{#1}{#2}{#3}}}
%
\def \derLmuFour #1 |- #2 : #3 | #4 {\hskp {#1} \TurnLmu \Stoup{#2}{#3} \Mid {#4} \hskp}
\def \derLmuNormal #1 |- #2 : #3 {\@ifnextchar|{\derLmuFour #1 |- #2 : #3 }{#1 \TurnLmu \Stoup{#2}{#3} }}
\def \derLmuCmd #1 |- #2 | #3 {\hskp {#1} \TurnLmu {#2} \Mid {#3} \hskp }
\def \derLmuBasis #1 |- #2 {\@ifnextchar:{\derLmuNormal #1 |- #2 }{\derLmuCmd #1 |- #2 }}
\def \derLmu {\@ifnextchar|{\derLmuBasis {} %{\emptyset}
	 }{\derLmuBasis }}
\def \derLmuP {\def \Turn {\TurnP}\derLmu}
\def \derLmuR {\def \Turn {\TurnR}\derLmu}
\def \derLmuO {\def \Turn {\mathrel{\vdash}}\derLmu}
\def \derL #1 |- #2 : #3 {{#1} \TurnL {#2} : {#3}}

\def \Der{{\cal D}}

\def \modelsLmu #1 |- #2 : #3 | #4 {\hskp {#1} \models \Stoup{#2}{#3} \Mid {#4} \hskp}
\def \Models{\models}

\def \bottom{{\perp}}
\def\dquad{\quad\quad}
\def\qquad{\dquad\dquad}
\def\Stat #1:{#1{:}}
\def \Red{}
\def \lterm{}
\def \lmmt	{{\Red \overline{`l}`m\tilde{\mu}}}
\def \MIU {{\Red \cal M^{\cap\cup}}}
\def \Lmu{`l`m}
\def \LK{\textsc{lk}}
\def \X {{\cal X}}
\def \unI	{{\Red \cup \textsl{I}}}
\def \unE	{{\Red \cup \textsl{E}}}
\def \seq {\mathrel{\leq}}
\def \seqC {\mathrel{\leq_C}}
\def \seqD {\mathrel{\leq_D}}
\def \filt{{\uparrow}\skp}
\def \TL#1{\overline{#1}}
\def \TR#1{\underline{#1}}

\def \dblambda  {\psset{unit=1\point,linewidth=.75\point}%
\kern3\point
\psline{-}(.9,0.45)(2,.8)%
\psline{-}(1.75,.55)(2.1,2.1)%
\kern-2.8\point\lambda \kern-.5em\raise.15em\hbox{$\lambda$}\,}

\newcommand{\Abs}{\mbox{\it abs}}
\newcommand{\App}{\mbox{\it app}}
\newcommand{\Cut}{\mbox{\it cut}}
\newcommand{\False}{\bot}
\newcommand{\Name}{n}
\newcommand{\negI}{{\neg}I}
\newcommand{\negE}{{\neg}E}
\newcommand{\callCC}{{\cal C}}
\def\Rule(#1){(#1)}

\newskip \myitemmargin 

\def \myitem[#1]{\setbox55=\hbox{#1}\myitemmargin\wd55 
\advance\myitemmargin-\leftmarginii 
\item[{#1}]\leavevmode $ \kern -\myitemmargin  
\begin{array}[t]{@{}lclclclclcl} \kern \myitemmargin }

\def\LangR{\Lang_{\kern-.5\point\textsc {\scriptsize r}}}

%\def\ReplOne(#1){`x\skp#1}
\def\ReplOne(#1){`x\skp(#1)}
\def\Repl{\@ifnextchar({\ReplOne}{`x}}%)
\def\indexReplOne[#1]{\raise-2\point\hbox{\scriptsize $`x[#1]\kern1pt$}}
\def\indexRepl{\kern-1\point\@ifnextchar[{\indexReplOne}{\raise-2\point\hbox{\scriptsize $`x$}}}%]
%\def\indexRepl{_{`x}}

\def\dots{\cdots}
\def \black{}

 \newenvironment{AuxCases}[1]{\left \{ % \def\arraystretch{1.1} 
\begin{array}{#1} }{ \end{array} \right . }
 \renewenvironment{cases}{\@ifnextchar\bgroup{\begin{AuxCases}}{\begin{AuxCases}{@{\,}lclll}}}{\end{AuxCases}}

\def \Except	{{\setminus}}
\def \Redex{\mbox{\small \sf R}}
\def \RedP'{\mbox{\rm R'}}
\def \R {\@ifnextchar'{\RedP}{\Redex}}

\def \lored{\mathrel{\rightarrow_{\textit{\scriptsize lor}}}}
\def \Lor {\textsl{lor}\,}

\makeatother

% ] } )

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{S. Graham-Lengrand and L. Paolini (Eds.): Sixth Workshop on\\ Intersection Types and Related Systems (ITRS 2012).\\
EPTCS 121, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.121.1}{10.4204/EPTCS.121.1}}

